HMCF - Hamiltonian Monte Carlo Sampling for Fields - A Python framework for HMC sampling with NIFTy

HMCF "Hamiltonian Monte Carlo for Fields" is a software add-on for the NIFTy "Numerical Information Field Theory" framework implementing Hamiltonian Monte Carlo (HMC) sampling in Python. HMCF as well as NIFTy are designed to address inference problems in high-dimensional spatially correlated setups such as image reconstruction. HMCF adds an HMC sampler to NIFTy that automatically adjusts the many free parameters steering the HMC sampling machinery. A wide variety of features ensure efficient full-posterior sampling for high-dimensional inference problems. These features include integration step size adjustment, evaluation of the mass matrix, convergence diagnostics, higher order symplectic integration and simultaneous sampling of parameters and hyperparameters in Bayesian hierarchical models.

==> tex/demo_internet.tex <==
\subsection{German Internet}

In 1992 \todo{find correct date and source} the German internet providers
started to use the TV cable infrastructure to offer broadband connections for
most homes in Germany.

Because of the historic origin in TV signal distribution the cable net
infrastructure is mostly tree-like and for the scope of this example we simplify
this to a fully tree like system with different levels such as international
knots, federal knots and regional knots.
The main idea of this example is to find out whether a knot is malfunctioning,
based on incident reports from homes in Germany.

For our model we assume that every connection in Germany passes the
international \emph{commercial internet eXchange} knot $\eta^{(0)}_0$ in Frankfurt a.M.
(DE-CIX) and use this as the root of our tree (level 0).
$\eta^{(0)}_0$ is either $0$ if it is broken or $1$ if it works fine.
$20$ \emph{federal knots} $\eta^{(1)}_i$ (level 1) are connected directly to
this root knot (although there are only $16$ states in Germany).
Connected to the federal knots are thousands of \emph{regional knots}
$\eta^{(2)}$ which also define the smallest resolution for the origins of the
incident reports i.e., for each region $j$ the number of incidents $d_j$ is
reported.

We also assume that these regions are quadratic, have a population $N_j$ which is very
roughly proportional to the actual population and assume a constant rate
$\alpha$ throughout Germany of people who have a cable internet connection and
are willing to report incidents.
Additionally there is always a portion of people who report incidents which
actually have nothing to do with the knots but rather with inadequate router
setups in their homes.
We call this artifact the \emph{stupidity noise rate} $\beta$ and also assume
that this is a national problem and does not depend on the region.

Therefore the probability distribution for incidents by region $d_j$ is
Poissonian:
\begin{equation*}
  P(d_j | \lambda_j ) = \text{Poisson}(d_j ; \lambda_j)
\end{equation*}
where $\lambda_j = N_j (\alpha \omega_j + \beta)$.
Here $\omega_j$ is the binary variable stating whether the region $j$ has
internet access or not.
Its value can be formalized as
\begin{equation}\label{eq:regcon}
  \omega_j = \sum_{i,j} \eta^{(0)}_0 \cdot C^{(0)}_{0, i} \cdot \eta^{(1)}_i \cdot C^{(1)}_{i, j} \cdot \eta^{(2)}_j
\end{equation}
Where
\begin{equation*}
  C^{(l)}_{m, n} = \left\{  
  \begin{split}
    1, &\text{ if knot $m$ of level $l$ is connected to knot $n$ of level $l+1$} \\
    0, &\text{ else}
  \end{split}
  \right.
\end{equation*}
With equation (\ref{eq:regcon}) $\omega_j$ is either zero if at least one of the
knots connecting region $j$ to DE-CIX (or DE-CIX itself) is broken and one if
all connecting knots are working.

==> tex/demo_wiener_lognormal.tex <==
\subsection{Log Normal}
The Wiener filter example is nice as an proof of concept
but does not exactly show the advantages of an HMC approach.
The analytical solution calculated via conjugate gradients is essentially as fast as one
leapfrog integration step in the HMC approach and gives a nearly perfect solution.

To present a problem where an HMC approach is actually better
than other approaches we introduce a still rather simple
log-normal Wiener filter scheme.
Since there is no analytical solution for calculating the mean value
most algorithms calculate a maximum-a-posteriori (MAP) solution
which is most of the time good enough but does not in general
represent the actual mean value of the distribution.

In this example, again a Gaussian prior is set on $s$
\begin{equation}
  \Prob(s|S) \propto \exp \left( - \frac 12 s^\top S^{-1} s \right)
\end{equation}

but the data model for $d$ is changed to
\begin{equation}
  \label{eq:lndatagen}
  d = R e^s + n 
\end{equation}
with $n$ being Gaussian noise.
This imposes a log-normal prior on the variable $x = e^s$ implicitly.

The energy functional for the full posterior can be written as
\begin{equation}
  H(s|d) = \frac 12 s^\top S^{-1} s + \frac 12 (d - R e^s)^\top N^{-1}(d - Re^s) + \text{const}
\end{equation}

In this example we work on a (one-dimensional) 1024 pixel regular space
to keep the sampling time relatively short.

Once again the covariance $S$ is assumed to be diagonal in the harmonic space of $s$
with its power spectrum given by (\ref{eq:powspec}).

\subsubsection[Implementation in \purehmcif]{Implementation in \hmcif}
The following code snippets can also be found in the \hmcif\ package's demo
folder in the nonlinear\_wiener\_filter\_demo.py script.
A similar demo is also available in \nifty\ solving the problem with a
MAP algorithm.
In the \hmcif\ demo we use the MAP solution to compare our mean solution to.

The demo works by default on a (one-dimensional) 1024 pixel regular space.
For simplicity we assume again that for the following example $D$, $S$, $R$ and $N$
are already well defined as \niftyo s.
But our instrument $R$ is broken in that it has a blind spot 200 pixels wide where it only
returns zeros to make the problem a little more interesting.

As in the case of the Wiener filter example a \niftyo\ defined as \code{HT}
transforms fields from the harmonic to the position representation.
We further introduce a field $\powvar = \text{diag}(S)^{\frac 12}$
which imprints the power spectrum in the harmonic representation of $s$ onto a
white noise field.
With that we can introduce a new random variable $z = \powvar^{-1} \odot s$
($\odot$ represents the Hadamard Product) for sampling which has the identity as prior covariance since
\begin{equation}
  s^\top S^{-1}s = (\powvar^{-1}\odot s)^\top (\powvar^{-1} \odot s) = z^\top z   .
\end{equation}
The field representation of $z$ is the prior eigenbasis.

Sampling in the space of $z$ but being interested in $e^s$ also means that we need a non-linear transformation
of our samples before expectation values can be calculated:
\begin{CodeChunk}
  \begin{CodeInput}
  import nifty4 as ift
  import hmcf
  [...]
  non_linearity = ift.library.nonlinearities.Exponential()
  [...]
  def sample_transform(z):
    return non_linearity(HT(power*z))
  \end{CodeInput}
\end{CodeChunk}

The energy for the full posterior in equation (\ref{eq:wiener}) is already
implemented as \eon\ in \nifty .
First we use the MAP approach of \nifty\ for comparison:
\begin{CodeChunk}
  \begin{CodeInput}
  m = ift.Field.full(h_space, 1e-7)
  posterior_energy = ift.library.NonlinearWienerFilterEnergy(
      m, d, R, non_linearity, HT, power, N, S, inverter=inverter)

  # Minimization with chosen minimizer
  posterior_energy = minimizer(posterior_energy)[0]
  map_solution = posterior_energy.position
  \end{CodeInput}
\end{CodeChunk}
where \code{minimizer} is an \nifty\ algorithm returning an \eon\
at the MAP position.

As starting points for our Markov chains we create samples from the
prior covariance $S$ (still the identity) with mean \code{map_solution}:
\begin{CodeChunk}
  \begin{CodeInput}
  x_initial = [map_solution + S.draw_sample() for _ in range(num_processes)]
  \end{CodeInput}
\end{CodeChunk}

Creating an \hmcsc\ instance and adjusting some parameters works as before
with the Wiener filter:
\begin{CodeChunk}
  \begin{CodeInput}
  nl_hmc = hmcf.HMCSampler(potential=posterior_energy,
                          num_processes=num_processes,
                          sample_transform=sample_transform)
  nl_hmc.display = hmcf.TableDisplay
  nl_hmc.epsilon = hmcf.EpsilonPowerLawDivergence
  nl_hmc.mass.reevaluations = 3
  nl_hmc.run(num_samples=1000, max_burn_in=5000,
             convergence_tolerance=1.,
             x_initial=x_initial)
  \end{CodeInput}
\end{CodeChunk}

\subsubsection{Results}
Afterwards the HMC mean is compared to the MAP solution of the problem:
\begin{CodeChunk}
  \begin{CodeInput}
  hmc_mean = nl_hmc.mean
  hmc_std = ift.sqrt(nl_hmc.var)
  map_solution = sample_transform(map_solution)
  diff = abs(map_solution - hmc_mean)
  \end{CodeInput}
\end{CodeChunk}
and again visualized:
\begin{CodeChunk}
  \begin{CodeInput}
  lo = np.min([true_sky.min(), map_solution.min(), data.min()])
  hi = np.max([true_sky.max(), map_solution.max(), data.max()])
  plotdict = {"colormap": "Planck-like", "ymin": lo, "ymax": hi}
  ift.plot(true_sky, name="true_sky.png", **plotdict)
  ift.plot(map_solution, name="reconstructed_sky.png", **plotdict)
  ift.plot(data, name="data.png", **plotdict)
  ift.plot(hmc_mean, name='hmc_mean.png', **plotdict)
  ift.plot(diff, name='difference.png', **plotdict)
  ift.plot(hmc_std, name='hmc_std.png', colormap="Planck-like",
           ymin=0., ymax=hmc_var.max())
  \end{CodeInput}
\end{CodeChunk}
These images generated with \code{numpy.random.seed(42)} are depicted in figure
\ref{fig:lndemo}.

\begin{figure}
  \captionsetup[subfigure]{oneside,margin={-2cm,0cm}}
 
\begin{subfigure}{0.5\textwidth}
\includegraphics{log_normal/mock_signal} 
\caption{true signal}
\label{fig:lnsig}
\end{subfigure} 
\begin{subfigure}{0.5\textwidth}
\includegraphics{log_normal/data} 
\caption{data field}
\label{fig:lndata}
\end{subfigure}

\begin{subfigure}{0.5\textwidth}
\includegraphics{log_normal/hmc_mean} 
\caption{HMC mean}
\label{fig:lnhmc}
\end{subfigure} 
\begin{subfigure}{0.5\textwidth}
\includegraphics{log_normal/map_sol} 
\caption{MAP solution}
\label{fig:lnmap}
\end{subfigure}

\begin{subfigure}{0.5\textwidth}
\includegraphics{log_normal/hmc_var} 
\caption{HMC std}
\label{fig:lnhmcvar}
\end{subfigure} 
\begin{subfigure}{0.5\textwidth}
\includegraphics{log_normal/difference} 
\caption{difference}
\label{fig:lndiff}
\end{subfigure} 

\caption{Results of the log\_normal\_demo.py script.
  It shows that the MAP solution (figure \subref{fig:lnmap}) is in this case a very
  good approximation to the true (HMC) mean (figure \subref{fig:lnhmc}).
  The HMC mean was calculated using in total 5000 samples.
  The problem includes a partially 'broken' instrument
  which can be easily seen as a prominent zero-valued feature in
  the data field (figure \subref{fig:lndata}).
  In figure \subref{fig:lnhmcvar} the high uncertainty of the HMC sampler in
  this region can be observed.}
\label{fig:lndemo}
\end{figure}



==> tex/demo_wiener_simple.tex <==
\subsection{Wiener Filter}
A rather easy inference problem assuming that a measurement with an instrument
provides a data field $d$ with the stochastic equation
\begin{equation}\label{eq:data}
  d = Rs + n
\end{equation}
where $n$ is Gaussian white noise (covariance $N$) and $s$ the signal.
$R$ is a linear operator representing the instrument's response.

If $s$ has a Gaussian prior with covariance $S$ one can show that the
full posterior is
\begin{equation}\label{eq:wiener}
  \begin{split}
  \Prob(s|d) &\propto \exp \left( -\frac 12 s^\top S^{-1} s - \frac 12 (d - Rs)^\top N^{-1}(d - Rs) \right)\\
         &\propto \exp \left( -\frac 12 (s-m)^\top D^{-1}(s-m) \right)
  \end{split}
\end{equation}
where $D^{-1} = S^{-1} + R^\top N^{-1} R$ and $m = DR^\top N^{-1}d$ the
mean value.

The advantage of choosing this problem is that there exists a analytic solution
for the mean value $m$ and therefore a comparable solution for the HMC sampler.

We assume the covariance $S$ to be diagonal in the harmonic representation
of the space for $s$ with a power spectrum $\P(k)$:
\begin{equation}
  \label{eq:powspec}
  P(k) \propto \left( 1 + \frac kk_0 \right)^{-4}
\end{equation}
where $k_0$ defines the correlation length.
Furthermore the signal-to-noise ratio (SNR) is 1,
meaning that the covariance of $n$ is roughly as big as the (mean) variance
of $s$ in the position space.

\subsubsection[Implementation in \purehmcif]{Implementation in \hmcif}
The following code snippets can also be found in the \hmcif\ package's demo
folder in the wiener\_filter\_demo.py script.
A full Wiener filter demo (without HMC sampling) can also be found in the \nifty\ package.

The demo works by default on a 64x64 pixel regular space
with the covariance of the signal $s$ being given as described above.
This means that there are 4,096 degrees of freedom.
For simplicity assume that for the following example $D$, $S$, $R$ and $N$
are already well defined as \niftyo s.
Also our data field $d$ is available as \niftyf .

Since $S$ is only diagonal in the harmonic space the sampling itself
takes place in that representation.
Another \niftyo\ defined as \code{HT} transforms fields from the harmonic
to the position representation.
The energy for the full posterior in equation (\ref{eq:wiener}) is already
implemented as \eon\ in \nifty , too.

With that an \hmcsc\ instance can be defined as:
\begin{CodeChunk}
  \begin{CodeInput}
  import nifty4 as ift
  import hmcf
  [...]
  posterior_energy = ift.library.WienerFilterEnergy(position=start_position,
                                                    d=d, R=R, N=N, S=S,
                                                    inverter=inverter)
  wiener_hmc = hmcf.HMCSampler(potential=posterior_energy, num_processes=5,
                              sample_transform=HT)
  \end{CodeInput}
\end{CodeChunk}
where \code{start_position} is just a field in the harmonic representation of
the space for $s$ with zero value everywhere.
The \code{inverter} is a tool in \nifty\ for numerically inverting operators.

To optimize the sampling process additional features are set:
\begin{CodeChunk}
  \begin{CodeInput}
  wiener_hmc.epsilon = hmcf.EpsilonPowerLaw
  wiener_hmc.mass.reevaluations = 2
  wiener_hmc.display = hmcf.TableDisplay
  \end{CodeInput}
\end{CodeChunk}

And finally a run is initiated:
\begin{CodeChunk}
  \begin{CodeInput}
  wiener_hmc.run(num_samples=200, convergence_tolerance=0.5)
  \end{CodeInput}
\end{CodeChunk}

\subsubsection{Results}
Afterwards the HMC mean is compared to the analytic solution of the problem:
\begin{CodeChunk}
  \begin{CodeInput}
    hmc_mean = wiener_hmc.mean
    analytic_mean = HT(D*R.adjoint*N.inverse(d))
    diff = abs(hmc_mean - analytic_mean)
  \end{CodeInput}
\end{CodeChunk}
and visualized using the \nifty\ plot functions:
\begin{CodeChunk}
  \begin{CodeInput}
    lo = hmc_mean.min()
    hi = hmc_mean.max()
    plotdict = {"colormap": "Planck-like", "ymin": lo, "ymax": hi}
    ift.plot(hmc_mean, name="hmc_mean.png", **plotdict)
    ift.plot(analytic_mean, name="analytic_mean.png", **plotdict)
    ift.plot(diff, name='difference.png', **plotdict)
  \end{CodeInput}
\end{CodeChunk}

When running the script the HDF5 file is saved to a
(new) subdirectory ``samples'' where the script is located.

Additionally the last lines in the code above generate plots using the
\python\ package \pkg{matplotlib} in the directory from
where the script was started.

Figure \ref{fig:wienerdemo} displays these plots generated
using \code{numpy.random.seed(42)}.

\begin{figure}[ht]
  \captionsetup[subfigure]{oneside,margin={-2cm,0cm}}
 
\begin{subfigure}{0.5\textwidth}
\includegraphics{wiener_filter/hmc_solution} 
\caption{}
\label{fig:wienerhmc}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics{wiener_filter/analytical_solution}
\caption{}
\label{fig:wienerana}
\end{subfigure}
 
\begin{subfigure}{0.5\textwidth}
\includegraphics{wiener_filter/difference} 
\caption{}
\label{fig:wienerdiff}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics{wiener_filter/data}
\caption{}
\label{fig:wienerdata}
\end{subfigure}
 
\caption{Results of the wiener\_filter\_demo.py script.
  The first row represents the two approaches in solving the problem,
  where \subref{fig:wienerhmc} is the mean of the HMC samples and
  \subref{fig:wienerana} the conjugate gradient solution.
  In the bottom row the absolute difference of both approaches is
  displayed in \subref{fig:wienerdiff}
  and finally in \subref{fig:wienerdata} the mock data field from
  which the reconstruction was performed.}
\label{fig:wienerdemo}
\end{figure}



==> tex/symplectic_integrators.tex <==
\section{Symplectic Integrators}\label{sec:sympintegr}
\todo{reference the point where higher orders can be set in HMCF}

One of the most challenging tasks when implementing HMC is to solve Hamilton's
equations (\ref{eq:hamiltondyn}).
Fortunately solving Hamilton's equations is very central to modern Physics.
Therefore literature on numerical integrators tackling Hamiltonian dynamics
is quite broad and advanced (see e.g. \cite{leimkuhler2004, sympintegr01, 
sympintegr02}).
One very important class of such integrators are symplectic integrators which
keep the volume preserving property of Hamiltonian dynamics.
This section is supposed to give some intuition on how symplectic integrators
are derived and follows largely \cite{leimkuhler2004}. 

We start with decomposing the Hamiltonian $H$ into two
pseudo-Hamiltonians $H_1$ and $H_2$:
\begin{equation*}
  H(x, p) = \frac 12 p^\top M^{-1} p + V(q), ~~H_1(q, p) = \frac 12 p^\top M^{-1} p, ~~H_2(q, p) = V(q)
\end{equation*}
Let $\Phi_{\epsilon, H_i}$ be the map projecting a position $(q, p)$ 
forward in time by $\epsilon$ according to the Hamiltonian $H_i$.
The dynamics can be derived exactly for each of these:
\begin{align*}
  \Phi_{\epsilon, H_1} (q, p) &= \twovector{q + \epsilon \nabla_p K(p)}{p}\\
  \Phi_{\epsilon, H_2} (q, p) &= \twovector{q}{p - \epsilon \nabla_q V(q)}
\end{align*}
Since these maps depict Hamilton's equations exactly,
they preserve volume and are therefore symplectic.
Additionally since the composition of two symplectic maps is again symplectic,
the map
\begin{equation*}
  \Psi_{\epsilon} = \Phi_{\epsilon, H_1} \circ \Phi_{\epsilon, H_2}
\end{equation*}
is symplectic, too.
It remains to show that $\Psi_{\epsilon}$ approximates the true Hamiltonian
dynamics, represented by the map $\Phi_{\epsilon}$ as introduced in (\ref{eq:phih}).
A look at the behavior of $\Psi_{\epsilon}$ reveals
\begin{align}\label{eq:symplecticone}
  \Psi_{\epsilon}(q, p) &= \Phi_{\epsilon, H_1}(\Phi_{\epsilon, H_2}(q, p)\nonumber\\
    &= \Phi_{\epsilon, H_1}(q, p + \epsilon \nabla_q V(q))\nonumber\\
    &= \twovector{q}{p} + \epsilon \twovector{\nabla_{p^\prime} K(p^\prime)}{- \nabla_q V(q)}
\end{align}
where $p^\prime = p + \epsilon \nabla_q V(q)$.
On the other hand a Taylor expansion of $\Phi_{\epsilon}$ to first order in $\epsilon$ reads
\begin{equation*}
  \Phi_{\epsilon} = \twovector{q}{p} +\epsilon \twovector{\nabla_p}{-\nabla_q} H(q, p)  + \mathcal{O}({\epsilon}^2)
\end{equation*}
which shows immediately that $\Psi_{\epsilon}$ approximates the true
Hamiltonian dynamics up to first order in $\epsilon$.

But the volume preserving property of Hamiltonian dynamics is not the only neat
 side effect when using it in the context of MCMC algorithms.
For example the time-reversal property is necessary to ensure detailed balance.
Therefore it is necessary to impose an additional ``symmetry'' condition
on the symplectic integrator:
\begin{equation*}
  \Psi_{\epsilon} =  \Psi^\dagger_{\epsilon}
\end{equation*}
Where the adjoint map $\Psi^\dagger_{\epsilon}$ is defined as
\begin{equation*}
  \Psi^\dagger_{\epsilon} = \left( \Psi_{- \epsilon} \right)^{-1} \quad . 
\end{equation*}
In other words: For a symmetric symplectic integrator $\Psi_{\epsilon}$ the
inverse is just the same transformation propagating backwards in time by
$\epsilon$.

It is easy to see that if a numerical method as well as its adjoint map are known 
a symmetric method is available as
\begin{equation}\label{eq:symmetriccomp}
  \hat \Psi_{\epsilon} = \Psi_{\epsilon /2}^\dagger \circ \Psi_{\epsilon /2}
\end{equation}
The integrator presented in (\ref{eq:symplecticone}) for example is in general
not symmetric.
But the $\Phi_{\epsilon, H_i}$ are and therefore the adjoint of
(\ref{eq:symplecticone}) is given by 
\begin{align*}
  \Psi_\epsilon^\dagger &= \left( \Phi_{\epsilon, H_1} \circ \Phi_{\epsilon, H_2} \right)^\dagger\\
    &= \Phi_{\epsilon, H_2}^\dagger \circ \Phi_{\epsilon, H_1}^\dagger\\
    &= \Phi_{\epsilon, H_2} \circ \Phi_{\epsilon, H_1} \quad . 
\end{align*}
Using (\ref{eq:symmetriccomp}) a symmetric integrator can be constructed
which reads:
\begin{align}\label{eq:leapfrogpsi}
   \hat \Psi_\epsilon &= \Phi_{\epsilon /2, H_2} \circ \Phi_{\epsilon /2, H_1} \circ
     \Phi_{\epsilon /2, H_1} \circ \Phi_{\epsilon /2, H_2}\nonumber\\
     &= \Phi_{\epsilon /2, H_2} \circ \Phi_{\epsilon, H_1} \circ \Phi_{\epsilon /2, H_2}
\end{align}
where the second equality holds since the shift introduced by $\Phi_{\epsilon
  /2, H_1}$ is only dependent on $p$ and only changes $q$.
This is the well known leapfrog integrator as can be seen when applying it to a
state $(q(t), p(t))$:
\begin{equation}\label{eq:leapfrog}
\begin{split}
 p(t+\epsilon /2) &= p(t) - \frac \epsilon 2 \nabla_q V(q(t))\\
 q(t+ \epsilon ) &= q(t) + \epsilon \nabla_p K(p(t+\epsilon /2))\\
 p(t+ \epsilon ) &= p(t+\epsilon /2) - \frac\epsilon 2 \nabla_q V(q(t+\epsilon ))
\end{split}
\end{equation}
It can be shown that the leapfrog integrator approximates the true
Hamiltonian flow up to second order in $\epsilon$ exactly \cite{leimkuhler2004}.
The leapfrog integrator is the most used integrator for HMC sampling.
For evolving the system in time by $\tau$ the integration consists of $L$
successive applications of leapfrog steps such that $\tau = \epsilon L$.
The whole integration is of order 1 \cite{leimkuhler2004}.

\subsection{Higher Order Symplectic Integrators}
In principle one is not bound to second order integrators.
Higher order integrators can have better performance on high-dimensional spaces
\citet{higherordersymp01, higherordersymp02}.
The splitting of the Hamiltonian into potential $V$ and kinetic term $K$ can be
generalized to
\begin{equation*}
  H = \sum_{i=1}^k c_i K + \sum_{i=1}^k d_i V 
\end{equation*}
where $c_i$ and $d_i$ are normalized weights.
This leads to a symplectic map of the form
\begin{equation*}
  \hat \Psi_\epsilon =  \Phi_{c_1\epsilon , K} \circ \Phi_{d_1\epsilon, V} \circ
    \Phi_{c_2\epsilon, K} \circ \Phi_{d_2\epsilon, V} \circ \ldots
\end{equation*}
Although in principle the weights can be chosen arbitrarily the main idea of
further splitting the Hamiltonian is to generate higher or in particular
$k$-order symplectic integrators.
This means that $c_i$ and $d_i$ should ideally be chosen such that
the final symplectic map $\hat \Psi_\epsilon$ equals the Taylor expansion of
$\Phi_{\epsilon, H}$ up to order $k$ in $\epsilon$ while maintaining symmetry.
This is a very non-trivial task and it is hopeless to get higher order integrators by brute force methods \citep{neri1987}. 
\cite{yoshida1990} developed a method to derive higher order methods
by using known lower order expressions such as (\ref{eq:leapfrogpsi}).
Under the assumption a symmetric integrator $\hat \Psi_{\epsilon}^{(2k)}$
of order $2k$ is known, a symmetric
integrator of order $2(k+1)$ is constructed via
\begin{equation*}
  \hat \Psi_{\epsilon}^{(2(k+1))} = \hat \Psi_{\omega_0\epsilon}^{(2k)} \circ
    \hat \Psi_{\omega_1\epsilon}^{(2k)} \circ \hat \Psi_{\omega_2\epsilon}^{(2k)}
\end{equation*}
where the $\omega_i$s are again normalized weights.
For the integrator to be symmetric the condition $\omega_0 = \omega_2$ must hold.
Additionally normalizing gives
\begin{equation*}
  \omega_1 = 1 - 2\omega_0 \quad .
\end{equation*}
A third condition on the weights is given by the requirement that the
symplectic integrator needs to be equal to the Taylor expansion of
$\Phi_{\epsilon, H}$ up to order $2(k+1)$.
\cite{yoshida1990} derives the condition
\begin{equation*}
  \omega_1^{2k+1} + 2\omega_0^{2k+1} = 0
\end{equation*}
by making use of an alternative approach using Poisson brackets and the 
Baker-Campbell-Hausdorff formula.
The analytical solution for the weights of a $2(k+1)$-order integrator
is given by
\begin{equation*}
  \begin{split}
    \omega_0 &= \frac{1}{2-2^{1/(2k+1)}}\\
    \omega_1 &= - \frac{2^{1/(2k+1)}}{2-2^{1/(2k+1)}}\\
  \end{split}
\end{equation*}

In principal this enables the creation of integrators of arbitrary high order.
A drawback is that the number of intermediate steps grows exponentially with
$3^{k-1}+1$ for an $2k$ order integrator. 
Although there are approaches (without analytical solutions for the weights)
which get rid of the exponential scaling \cite{yoshida1990}, they would go beyond the scope of this
work.

